Measuring Optical Extinction Towards Young Stellar Objects Using Diffuse Interstellar Bands

Line-of-sight extinction estimates to well-studied young T Tauri and Herbig Ae/Be stars are based on many different measurements and analysis methods. This has resulted in wide scatter among the published $A_V$ values for the same star. In this work, we discuss the challenges in measuring extinction to actively accreting and especially outbursting young stellar objects (YSOs). We then explore a method not previously applied to young stars utilizing diffuse interstellar bands (DIBs). In early-type stars, narrow correlations exist between DIB equivalent widths and the column density of interstellar material, and therefore the line-of-sight extinction. Here, we measure equivalent widths of the 5780 \AA\ and 6614 \AA\ DIB features in a sample of actively accreting YSOs, and apply a DIB-reddening calibration to estimate reddening and subsequently extinction. Our calibration is newly derived from a composite of available literature data and fully accounts for the scatter in these measurements. We also compare the DIBs-inferred optical line-of-sight extinction values with previous extinction estimates for our sample stars.

==> table3_backup.tex <==
% THIS IS A COPY MADE 20220904 BEFORE FINAL EDITING


\begin{longrotatetable}
\begin{deluxetable*}{c|cc|cc|ccc|cc|cc}
	\tablecaption{Literature properties of outbursters in our sample.\label{tab:OutburstersProperties}}
	\tablewidth{0pt}%700
	\tablehead{
	    \colhead{Target} & \colhead{System RV} & 
		\colhead{Ref} & \colhead{SpT} & \colhead{Ref} & \colhead{$A_V$} & \colhead{Ref} & \colhead{$A_V$ (X-Ray) \tablenotemark{a}} & \colhead{$L_{\text{quiescent}}$} & \colhead{Ref} & \colhead{$L_{\text{burst}}$} & \colhead{Ref} 
	}
	\startdata
	\multicolumn{12}{c}{Young Star Outbursters } \\
    \hline
    BBW 76 & 30 & 5 & G0-G2\tablenotemark{b} \& K/M\tablenotemark{g} & 5 & 2.1 & 5 & $\cdots$ & $\cdots$ & $\cdots$ & 453\tablenotemark{i} & 5 \\
    FU Ori & 28 & 6 & G0 & 8 & 1.4 & 6 & 81 & $\cdots$ & $\cdots$ & 66 & 4 \\
    Gaia 17bpi & 4.5 & 10 & GK\tablenotemark{d}\tablenotemark{g} & 10 & 3 & 10 & 4.1 & 0.3 & 10 & 7.5 & 10 \\
    Gaia 19ajj & 35.8 & 26 & M3 & 26 & 6 & 26 & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ \\
    V899 Mon & 0.92 & 3 & $\cdots$ & $\cdots$ & 2.6-4.5 & 3 & $\cdots$ & 162 & 3 & 419 & 3 \\
    LkHa 225 S & -13.5 & 32 & A2V\tablenotemark{e} & 9 & 7.2 & 9 & $\cdots$ & $\cdots$ & $\cdots$ & 750 & 9 \\
    V960 Mon & 38.1 & 14 & G2-K1 & 11 & 1.5 & 4 & 2.6 & 4.8 & 15 & 48 & 4 \\
    PTF 10qpf & ~1.6 & 13 & K7III\tablenotemark{g, e} \& K7-M0 \tablenotemark{f} & 12 & 3.4 & 16 & 4.1 & 2.69 & 16 & 12 & 13 \\
   %PTF 15afq & $\cdots$ & $\cdots$ & T=9620K & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & 111 & 2 \\
    PTF 15afq & $\cdots$ & $\cdots$ & F5-G0 & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & 111 & 2 \\
    RNO 1B & $\cdots$ & $\cdots$ & F8II & 27 & 14.5 & 4 & $\cdots$ & 527 & 28 & 1652 & 4 \\
    V582 Aur & $\cdots$ & $\cdots$ & G0I\tablenotemark{e} & 19 & 6.5,5.6 & 18,4 & $\cdots$  & $\cdots$ & $\cdots$ & 500-1050\tablenotemark{j} & 18\\
    V733 Cep & $\cdots$ & $\cdots$ & G5-6Ib\tablenotemark{b}\tablenotemark{g} & 30 & 11.5 & 4 & $\cdots$  & $\cdots$ & $\cdots$ & 43\tablenotemark{k} & 4\\
    V1057 Cyg & -16 & 6 & F7-G3 & 6 & 2.4-3.9 & 6,4 & 4.1  & $\cdots$ & $\cdots$ & 100\tablenotemark{l} & 4 \\
    V1331 Cyg & $\cdots$ & $\cdots$ & F0-F4/G5 & 20,21 & 2.4 & 25 & $\cdots$ & $\cdots$ & $\cdots$ & 53 & 22 \\
    V1515 Cyg & -12 & 23 & G2-G5 & 24 & 3.5 & 4 & 4.1 & $\cdots$ & $\cdots$ & 103-200 & 6,22 \\
    V900 Mon & $\cdots$ & $\cdots$ & 6400K & 21 & 13.5 & 4 & 4.1 & $\cdots$ & $\cdots$ & 99 & 4 \\
    Z CMa & -30 & 33 & 6500K & 21 & 7.1 & 4 & 4.1 & $\cdots$ & $\cdots$ & 3548\tablenotemark{m} & 4 \\
    \hline
    \multicolumn{12}{c}{Other Photometric Variables with DIBs } \\
    \hline
    ASASSN 15qi & -58.1 & 1 & F8 & 7 & 3.6 & 7 & $\cdots$ & 18 & 7 & 1000 & 7 \\
    PTF 14jg & -38.1 & 17 & A \tablenotemark{b} \& late F \tablenotemark{c} \& G-K \tablenotemark{d}  & 17 & 4.75 & 17 &  0.1-0.3 & $\cdots$ & $\cdots$ & 130 & 17  \\
    PTFS1821n & $\cdots$ & $\cdots$ & B1\tablenotemark{h} & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ \\
    RNO 1A & 6.61 & 29 & F5III\tablenotemark{*} & 27 & 3.6 & 27 & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ \\
    VES 263 & -4.1 & 31 & B1 & 31 & 5.6 & 31 & $\cdots$ & 14000 & 31 & $\cdots$ & $\cdots$ \\
\enddata
    \tablecomments{Literature Sources: (1) \citet{hillenbrand_optical_2015}, (2) \citet{sewilo_identifying_2019}, (3) \citet{ninan_v899_2015}, (4) \citet{connelley_near-infrared_2018}, (5) \citet{reipurth_evolution_2002}, (6) \citet{herbig_high-resolution_2003}, (7) \citet{herczeg_eruption_2016}, (8) \citet{kenyon_flickering_2000}, (9) \citet{magakian_new_2019}, (10) \citet{hillenbrand_gaia_2018}, (11) \citet{park_high-resolution_2020}, (12) \citet{fang_first_2020}, (13) \citet{miller_evidence_2011}, (14) \citet{takagi_spectroscopic_2018}, (15) \citet{kospal_progenitor_2015}, (16) \citet{cohen_observational_1979}, (17) \citet{hillenbrand_ptf14jg_2019}, (18) \citet{zsidi_weakening_2019}, (19) \citet{semkov_photometric_2013}, (20) \citet{chavarria-k_13-color_1981}, (21) \citet{gramajo_spectral_2014}, (22) \citet{sandell_similarity_2001}, (23) \citet{herbig_eruptive_1977}, (24) \citet{kolotilov_studies_1983}, (25) \citet{chavarria_study_1981}, (26) \citet{hillenbrand_gaia_2019}, (27) \citet{staude_rno_1991}, (28) \citet{skinner_chandra_2020}, (29) \citet{gaia_collaboration_gaia_2018}, (30) \citet{reipurth_v733_2007}, (31) \citet{munari_2018_2019}, (32) \citet{Hillenbrand_2022_lkha225s}, (33) \citet{SA2020}}
    \tablenotetext{*}{We derive a spectral type closer to A0 or F8 for RNO 1A, see Appendix \ref{appendix:rno1} for more details.}
    \tablenotetext{a}{$A_V$s from \citet{kuhn_comparison_2019}, derived from XMM-Newton X-Ray spectra or adopted for their analysis.}
    \tablenotetext{b}{According to characteristics of a blue spectrum}
    \tablenotetext{c}{According to characteristics of a green spectrum}
    \tablenotetext{d}{According to characteristics of a red spectrum}
    \tablenotetext{e}{Determined during an outbursting episode}
    \tablenotetext{f}{Determined during system quiescence}
    \tablenotetext{g}{Has M spectral type characteristics in the near-infrared.}
    \tablenotetext{h}{Determined by similarity to the optical spectrum VES 263 in the 5000-7500 \AA\ range.}
    \tablenotetext{i}{\citet{reipurth_evolution_2002} assume a distance of 1800 pc to the source. New Gaia parallax measurements give the distance to BBW 76 as 1092 pc, which decreases the value to 166 $L_\odot$}
    \tablenotetext{j}{Depending on the association, whether V582 Aur belongs to Auriga OB1 or Auriga OB2 \citep{zsidi_weakening_2019}}
    \tablenotetext{k}{Work by \citet{kuhn_comparison_2019} using Gaia DR2 parallaxes places V733 Cep at 825 pc, rather than 800 pc cited in \citet{connelley_near-infrared_2018}. The updated luminosity would be 40$L_\odot$.}
    \tablenotetext{l}{Work by \citet{kuhn_comparison_2019} using Gaia DR2 parallaxes places V1057 Cyg at 795 pc, rather than 550 pc cited in \citet{connelley_near-infrared_2018}. The updated luminosity would be 209$L_\odot$.}
    \tablenotetext{m}{Work by \citet{kuhn_comparison_2019} using Gaia DR2 parallaxes places Z CMa at 1120 pc, rather than 990 pc cited in \citet{connelley_near-infrared_2018}. The updated luminosity would be 4540$L_\odot$.}
\end{deluxetable*}
\end{longrotatetable}

